Three-loop contributions to the $\rho$ parameter and iterated integrals of modular forms

We compute fully analytic results for the three-loop diagrams involving two different massive quark flavours contributing to the $\rho$ parameter in the Standard Model. We find that the results involve exactly the same class of functions that appears in the well-known sunrise and banana graphs, namely elliptic polylogarithms and iterated integrals of modular forms. Using recent developments in the understanding of these functions, we analytically continue all the iterated integrals of modular forms to all regions of the parameter space, and in each region we obtain manifestly real and fast-converging series expansions for these functions.

==> Coaction.tex <==
\section{Symbol calculus and coaction for eMPLs}

\label{CoacSec}

In this section we are going to give a brief introduction to symbol calculus and coaction for the eMPLs, we choose an approach more focused on the application of these constructions and we refer to \cite{Broedel:2018iwv,BrownNMP} for a more detailed study.\par 
We first begin by making a comment about the meaning of the coaction and its importance in applications. When dealing with iterated integrals we would like often to search for different representations of the objects that we are handling or to look for identities among them. From a practical point of view, this need comes from the goal of reaching the simplest expression available for our result. In this context the coaction is a very powerful tool because it encodes, as the symbol map,  all the information about the differential structures of the iterated integrals but, unlike the symbol, it also also retains information about constants. It is then natural to use the coaction to relate different representations for iterated elliptic integrals and, as we will show explicitly, our final goal is precisely to use the coaction to obtain an expression for the elliptic master integral $f_7$ in terms of iterated integrals of modular forms. \par
We consider a generic iterated integral $\tilde{\Gamma}\left(\vec{A};z,\tau\right)$, where $\vec{A} = \left(A_1 \cdots A_k\right) = {\scriptsize\left(\begin{array}{ccc}
n_1 & \cdots & n_k \\ z_1 & \cdots & z_k
\end{array}\right)}$, and the vector
\be
\label{Jvec}
J = \left(J_{\vec{B}}\right)^T_{\vec{B} \in S} = \left(\int_0^z \Omega_{\vec{B}}\right)^T_{\vec{B} \in S}.
\ee
The entries of J are eMPLs which can be obtained by differentiating iteratively the integral $\tilde{\Gamma}\left(\vec{A};z,\tau\right)$, so loosely speaking the vector J is the vector of master integrals. The integrands $\Omega_{\vec{B}}$ can be written in terms of the integration kernels $g^{(n)}(z-\tau,\tau)$. Then the coaction acts on $\tilde{\Gamma}\left(\vec{A};z,\tau\right)$ as
\be
\label{eMPLsCoaction}
\Delta\left(\tilde{\Gamma}\left(\vec{A};z,\tau\right)\right) = \sum_{\vec{B} \in S} \tilde{\Gamma}\left(\vec{B};z,\tau\right) \otimes \mathscr S \left(\left[\Omega_{\vec{B}},\Omega_{\vec{A}}\right]\right),
\ee
where $\mathscr S \left(\left[\Omega_{\vec{B}},\Omega_{\vec{A}}\right]\right)$ is the symbol associated to a pair of differential forms.
 In the rest of this section we will introduce the elements needed to understand \ref{eMPLsCoaction} and we will highlight the main steps of its construction. Finally we will show an application of the coaction in the case of one of the iterated integrals on the torus involved in our computation.

\subsection{Total differential in the eMPLs case}

The first object that we need is an expression for the total differential in the eMPLs case, we limit ourselves to furnish the explicit formula and to describe its main features\footnote{A proof of the total differential formula can be found in \cite{Broedel:2018iwv}.}.\par
Given a certain iterated integral $\tilde{\Gamma}\left(A_1 \cdots A_k;z,\tau\right)$ the total differential is given by the formula
\bea
\label{dG}
&& d\tilde{\Gamma}\left(A_1\cdots A_k;z,\tau\right) = \sum_{p = 1}^{k-1}(-1)^{n_{p+1}}\tilde{\Gamma}{\scriptsize\left(A_1\cdots A_{p-1} \begin{array}{c}0 \\ 0\end{array}A_{p+2}\cdots A_k; z, \tau\right)} \omega_{p,p+1}^{(n_p + n_{p+1})} \nn \\
&& + \sum_{p = 1}^k\sum_{r = 0}^{n_p+1}\left[ {\scriptsize\left(\begin{array}{c} n_{p-1} + r -1 \\ n_{p-1} - 1\end{array}\right)}\tilde{\Gamma}{\scriptsize \left(A_1 \cdots A_{p-1}^{[r]} \hat{A}_p A_{p+1} \cdots A_k; z , \tau\right)}\omega_{p,p-1}^{(n_p - r)} \right. \nn \\
&& \left. - {\scriptsize\left(\begin{array}{c} n_{p+1} + r -1 \\ n_{p+1} -1 \end{array}\right)}\tilde{\Gamma}{\scriptsize \left(A_1 \cdots A_{p-1} \hat{A}_p A_{p+1}^{[r]}\cdots A_k;z,\tau\right)}\omega_{p,p+1}^{(n_p-r)}\right]
\eea
where $A_p^{[r]} \equiv {\scriptsize\left(\begin{array}{c} n_p + r \\ z_p \end{array} \right)}$, the hat means that the corresponding argument $\hat{A}_p$ is removed, and we use the conventions $\left(z_0,z_{k+1}\right) = (z,0)$, $(n_0,n_{k+1}) = (0,0)$.  The objects $\omega_{ij}^{(n)}$ are differential one-forms
\bea
\label{omegaF}
\omega_{ij}^{(n)} & = & (dz_j - dz_i)g^{(n)}(z_j - z_i, \tau) + \frac{n d\tau}{2\pi i}g^{(n+1)}(z_j - z_i,\tau), \;\;\; with \; n \geq 0, \nn \\
\omega_{ij}^{(-1)} & = & - \frac{d\tau}{2\pi i}.
\eea
From \ref{dG} it is possible to see that the action of the total differential lowers the length of the eMPLs by 1 and generates eMPLs of weight $k-1$. By acting iteratively with the total differential on the $k-1$ eMPLs generated at each step we build the vector of master integrals J in \ref{Jvec}.

\subsection{Motivic Coaction}

The next step for defining a coaction on eMPLs requires first a brief excursus on the notions of \emph{periods} and \emph{motivic periods}. Naively, we call period an integral $I = \int_{\gamma} \omega$ where the integrand is an algebraic function, and the domain is determined by algebraic inequalities, and motivic period the pair $[\gamma,\omega]$ where $\gamma$ is the integration path associated to $I$ and $\omega$ the differential form describing the integrand. (....)\par
Therefore we can define a kind of coaction which acts on motivic periods, which is called \emph{motivic coaction} \cite{BrownNMP} $\Delta^{\mathbf{m}}$, as
\be
\label{MotCoac}
\Delta^{\mathbf{m}} \left([\gamma,\omega]\right) = \sum_i [\gamma,\omega_i] \otimes [\omega_i, \omega]
\ee
Let us make some comments about \ref{MotCoac}.  The first entry of the motivic coaction is a motivic period $\left[\gamma,\omega_i\right]$ where the elements $\omega_i$ are a set of differential forms that describes the topology of the integral that we are considering, therefore we can think about them as master integrals and the sum in \ref{MotCoac} runs over the elements of the set $S$ in \ref{Jvec}. The second entry has a less obvious interpretation, indeed since it is a pair of differential forms $\left[\omega_i,\omega\right]$ it is not immediately clear if we can interpret it as an integral, like for the first entry, and therefore we do not know how to handle it. However, this apparent obstruction is precisely what lead us to the definition of coaction given in \ref{eMPLsCoaction}. Indeed, the idea is to define a symbol map for a pair of differential forms $\mathscr S \left(\left[\omega_i,\omega\right]\right)$ and then define the coaction on eMPLs as the composition
\be
\label{GenCoact}
\Delta \equiv (id \otimes \mathscr S)\Delta^{\mathbf{m}}.
\ee
In the following we are going to describe how to define a notion of symbol for a pair of differential forms.

\subsection{Symbol map for differential forms}

We consider the vector $J$ \ref{Jvec}, exploiting \ref{dG} by construction $J$ satisfies a linear differential equation of the first order 
\be
\label{JdiffEq}
dJ = AJ, \;\;\; with \;\;\; A = \sum_{i}A_i \omega_i.
\ee
Again, by construction the system \ref{JdiffEq} has a trivial homogeneous part and satisfies the integrability condition $dA = A \wedge A$, moreover the matrix $A$ is strictly upper triangular and therefore nilpotent.\par
Since the integrability condition is satisfied, eq. \ref{JdiffEq} admits a solution in terms of Chen-iterated integrals of the kind
\be
J(x) = \mathcal{W}(x)J_0
\ee
where $J_0$ is the vector of boundary conditions and $\mathcal{W}$ is defined as
\be
\mathcal{W} = \int_{\gamma} T_A, \; with \; T_A = 1 + [A]^R + [A\vert A]^R + \cdots [A^{k-1}]^R\;  and \; A^k =0.
\ee
Therefore the matrix $T_A$ encodes all the information about the iterative differential structure for the integrals vector $J$, this suggest the following definition for the symbol of a pair of differential forms:
\be
\label{SdiffForm}
\mathscr S (\left[\omega_i , \omega_j \right]) = \langle \omega_i \vert T_A \vert \omega_j \rangle = \left(T_A \right)_{ji}
\ee
In order to be properly defined the symbol map \ref{SdiffForm} has to satisfied all the usual properties of the symbol.(...)\par %%First of all, it is easy to see that \ref{SdiffForm} is bilinear:
%\be
%\mathscr S (\left[\omega_i + \omega_k, \omega_j\right]) = \langle \omega_i + \omega_k \vert T_A \vert \omega_j \rangle =  \langle \omega_i \vert T_A \vert \omega_j \rangle +  \langle \omega_k \vert T_A \vert \omega_j \rangle = \mathscr S (\left[\omega_i , \omega_j \right]) + \mathscr S (\left[\omega_k , \omega_j \right]).
%\ee
Before proceeding with an explicit example, we are going to make some general comments on the coaction. First, while the definition \ref{eMPLsCoaction} is for eMPLs, in general it is possible to construct a coaction starting the definition \ref{GenCoact} for any unipotent object, i.e. integrals that satisfy a differential equation of the kind \ref{JdiffEq} where $A$ is a nilpotent matrix. In particular it is possible to show \cite{Broedel:2018iwv} that the coaction in the MPLs case can be recovered from the same kind of construction used for the eMPLs case. A second comment, which is actually connected to the previous one,  regards the additional information that the coaction retains with respect to the symbol map. Let us consider the MPLs case, while the symbol maps to zero any constant term we can retain this lost information exploiting the coaction. In the eMPLs case we have a more complicated situation. As already said, the definition \ref{GenCoact} only makes sense for unipotent objects while often in computations involving eMPLs we have  handle quantities that are not unipotent. An example of this situation is given by the complete elliptic integrals of first and second kind $K(\lambda)$ and $E(\lambda)$, indeed they satisfy a coupled system of first order differential equation where the homogenous part is not trivial, and therefore the matrix $A$ is not nilpotent. To address this issue we can exploit the possibility to write a generic period $x$ as a linear combination
\be
x = \sum_i s_i u_i
\ee
where $u_i$ are unipotent periods and $s_i$ are called semi-simple periods \cite{BrownNMP}. Therefore we can define a coaction on semi-simple periods as
\be
\label{SemiSimpCoac}
\Delta(s_i) \equiv s_i \otimes 1.
\ee
This definition is consistent with the MPLs case, where the only semi-simple periods that appear are powers of $i \pi$, and extends the notion to elliptic case.

\subsection{Example}

We conclude this section discussing an explicit application of how the coaction can be used to rewrite an eMPLs in terms of iterated integrals of modular forms defined in \ref{IIh}. \par
We consider one of the eMPLs that appears in our computation for the master integral $f_7$:
\be
\label{Gex}
\tilde{\Gamma}{\scriptsize\left(\begin{array}{cc} 0 & 1 \\ 0 & \frac{2}{3}\end{array}; \frac{\tau}{2}, \tau\right)}.
\ee
The first step is to determined the vector $J$ of master integrals, this can be done by computing the total differential of \ref{Gex}. Using the formula \ref{dG} we get:
\bea
\label{GdG}
d \tilde{\Gamma}{\scriptsize\left(\begin{array}{cc} 0 & 1 \\ 0 & \frac{2}{3}\end{array}; \frac{\tau}{2}, \tau\right)} & = & - \tilde{\Gamma}{\scriptsize\left(\begin{array}{c} 0 \\ 0 \end{array};\frac{\tau}{2},\tau\right)}\omega^{(1)}_{1,2} + \sum_{r=0}^{1}\left[{\scriptsize\left(\begin{array}{c} r-1 \\ -1 \end{array}\right)}\tilde{\Gamma}{\scriptsize \left(\begin{array}{c} 1 \\ \frac{2}{3}\end{array}; \frac{\tau}{2},\tau \right)}\omega^{(-r)}_{1,0} - {\scriptsize \left(\begin{array}{c} r \\ 0 \end{array}\right)}\tilde{\Gamma}{\scriptsize \left(\begin{array}{c} 1 + r \\ \frac{2}{3}\end{array}; \frac{\tau}{2},\tau\right)}\omega^{(-r)}_{1,2}\right] \nn \\
&& + \sum_{r=0}^{2}\left[{\scriptsize\left(\begin{array}{c} r-1 \\ -1 \end{array}\right)}\tilde{\Gamma}{\scriptsize \left(\begin{array}{c} r \\ 0 \end{array}; \frac{\tau}{2},\tau \right)}\omega^{(1-r)}_{2,1} - {\scriptsize \left(\begin{array}{c} r -1 \\ -1 \end{array}\right)}\tilde{\Gamma}{\scriptsize \left(\begin{array}{c} 0 \\ 0 \end{array}; \frac{\tau}{2},\tau\right)}\omega^{(1-r)}_{2,3}\right]  = \nn \\
& = & \tilde{\Gamma}{\scriptsize \left(\begin{array}{c} 0 \\ 0 \end{array}; \frac{\tau}{2}, \tau\right)}\left[\omega_{2,1}^{(1)} - \omega_{2,3}^{(1)} - \omega_{1,2}^{(1)}\right] + \tilde{\Gamma}{\scriptsize \left(\begin{array}{c} 1 \\ \frac{2}{3} \end{array}; \frac{\tau}{2},\tau\right)}\left[\omega^{(0)}_{1,0} - \omega^{(0)}_{1,2}\right] - \tilde{\Gamma}{\scriptsize\left(\begin{array}{c} 2 \\ \frac{2}{3} \end{array}; \frac{\tau}{2}, \tau\right)}\omega^{(-1)}_{1,2} \nn \\
\eea
From this expression we can read off the vector $J$:
\be
J = \left(\tilde{\Gamma}{\scriptsize\left(\begin{array}{cc} 0 & 1 \\ 0 & \frac{2}{3}\end{array}; \frac{\tau}{2}, \tau\right)}, \tilde{\Gamma}{\scriptsize\left(\begin{array}{c} 0 \\ 0 \end{array}; \frac{\tau}{2}, \tau\right)},\tilde{\Gamma}{\scriptsize\left(\begin{array}{c} 1 \\ \frac{2}{3} \end{array}; \frac{\tau}{2}, \tau\right)}, \tilde{\Gamma}{\scriptsize\left(\begin{array}{c} 2 \\ \frac{2}{3} \end{array}; \frac{\tau}{2}, \tau\right)}, 1\right)^T.
\ee
In order to construct the full system of differential equation $D J = A J$ and obtain the matrix $A$ we have to compute also the total differential for length 1 eMPLs that appear in the vector $J$:
\bea
\label{GdGsub}
d \tilde{\Gamma}{\scriptsize\left(\begin{array}{c} 0 \\ 0 \end{array}; \frac{\tau}{2}, \tau\right)} & = & \omega^{(0)}_{1,0} - \omega^{(0)}_{1,2} \nn \\
d \tilde{\Gamma}{\scriptsize\left(\begin{array}{c} 1 \\ \frac{2}{3} \end{array}; \frac{\tau}{2}, \tau\right)} & = & \omega^{(1)}_{1,0} - \omega_{1,2}^{(1)} \nn \\
d \tilde{\Gamma}{\scriptsize\left(\begin{array}{c} 2 \\ \frac{2}{3} \end{array}; \frac{\tau}{2}, \tau\right)} & = & \omega^{(2)}_{1,0} - \omega^{(2)}_{1,2}
\eea
The differential one-forms $\omega^{(n)}_{ij}$ are given by the formula \ref{omegaF}:
\be
\begin{array}{cc}
\omega^{(0)}_{1,0} = \frac{d\tau}{2}; & \omega^{(0)}_{1,2} = 0 \\
\omega^{(-1)}_{1,2} = -\frac{d\tau}{2\pi i}; & \omega^{(1)}_{2,1} = \frac{d\tau}{2\pi i}g^{(2)}\left(-\frac{2}{3}; \tau\right) \\
\omega^{(1)}_{2,3} =  \omega^{(1)}_{2,1}; & \omega^{(1)}_{1,2} = \frac{d\tau}{2 \pi i}g^{(2)}\left(\frac{2}{3}; \tau\right) \\
\omega^{(1)}_{1,0} = \frac{d\tau}{2}g^{(1)}\left(\frac{\tau}{2} - \frac{2}{3};\tau\right) + \frac{d\tau}{2\pi i}g^{(2)}\left(\frac{\tau}{2} - \frac{2}{3};\tau\right); & \omega_{1,0}^{(2)} = \frac{d\tau}{2}g^{(2)}\left(\frac{\tau}{2} - \frac{2}{3};\tau\right) + \frac{d\tau}{\pi i}g^{(3)}\left(\frac{\tau}{2} - \frac{2}{3};\tau\right) \\
\omega^{(2)}_{1,2} = \frac{d\tau}{\pi i} g^{(3)}\left(- \frac{2}{3};\tau\right)
\end{array}
\ee
Therefore, from \ref{GdG},\ref{GdGsub} and from the definition of $J$ we see that the matrix $A$ is given by
\be
\label{A}
A = \left(\begin{array}{ccccc}
0 & \omega_{2,1}^{(1)} - \omega_{2,3}^{(1)} - \omega_{1,2}^{(1)} & \omega^{(0)}_{1,0} - \omega^{(0)}_{1,2} & -\omega^{(-1)}_{1,2} & 0 \\
0 & 0 & 0 & 0 &  \omega^{(0)}_{1,0} - \omega^{(0)}_{1,2}  \\
0 & 0 & 0 & 0 & \omega^{(1)}_{1,0} - \omega_{1,2}^{(1)} \\
0 & 0 & 0 & 0 & \omega^{(2)}_{1,0} - \omega^{(2)}_{1,2} \\
0 & 0 & 0 & 0 & 0
\end{array}\right).
\ee
At this point we are able to construct the matrix $T_A$. Since in this case $A^3 = 0$, $T_A$ we have
\be
T_A = 1 + [\, A ]\,^R + [\, A \vert A ]\,^R
\ee
where the non-zero elements, except the diagonal ones, are
\bea
\label{TA}
&&(T_A)_{1,2} = - [\, \omega^{(1)}_{1,2}]\, ; \;\;\;\; (T_A)_{1,3} = [\, \omega^{(0)}_{1,0} ]\, ; \;\;\;\; (T_A)_{1,4} = - [\, \omega^{(-1)}_{1,2}]\, ; \nn \\
&&(T_A)_{1,5} = - [\, \omega^{(0)}_{1,0} \vert \omega^{(1)}_{1,2}]\, + [\, \omega^{(1)}_{1,0} - \omega^{(1)}_{1,2}\vert \omega^{(0)}_{1,0}]\, - [\ \omega^{(2)}_{1,0} - \omega^{(2)}_{1,2} \vert \omega^{(-1)}_{1,2}]\, \nn \\
&&(T_A)_{2,5} = [\, \omega^{(0)}_{1,0}]\, ; \;\;\;\; (T_A)_{3,5} = [\, \omega^{(1)}_{1,0}]\, - [\, \omega^{(1)}_{1,2}]\, ; \;\;\;\; (T_A)_{4,5} = [\, \omega^{(2)}_{1,0}]\, - [\, \omega^{(2)}_{1,2} ]\,.
\eea
Finally, the last ingredient that we need to use the coaction and rewrite $\tilde{\Gamma}{\scriptsize\left(\begin{array}{cc} 0 & 1 \\ 0 & \frac{2}{3}\end{array}; \frac{\tau}{2}, \tau\right)}$ in terms of iterated integrals of modular forms is to express the integration kernels $g^{(n)}(a\tau + b; \tau)$ in terms of $h^{(n)}_{N,r,s}(\tau)$. Exploiting the relations \ref{gToH} we get the following expressions for the non-trivial differential one-forms $\omega^{n}_{ij}$:
\bea
\omega^{(1)}_{2,1} & = & \frac{d\tau}{2 \pi i}h^{(2)}_{6,2,0}(\tau), \nn \\
\omega^{(1)}_{1,0} & = & -\frac{i \pi d\tau}{4} - \frac{i d\tau}{2\pi}h^{(2)}_{6,2,3}(\tau) \nn \\
\omega^{(2)}_{1,0} & = & -\frac{\pi^2 d\tau}{12} - \frac{d\tau}{2} h^{(2)}_{6,2,3}(\tau) - \frac{i d\tau}{\pi}h^{(3)}_{6,2,3}(\tau) \nn \\
\omega^{(2)}_{1,2} & = & - \frac{i d\tau}{\pi} h^{(3)}_{6,2,0}(\tau).
\eea
Now, we are ready to use the coaction formula \ref{eMPLsCoaction} to rewrite \ref{Gex} in terms of iterated integrals of modular forms. Before proceeding to our example we discuss the general procedure. Let us consider a generic length $n$ eMPL, then  by looking at \ref{eMPLsCoaction} we see that in general we will have three kind of contributions to the coaction:
\be
\label{3TermsC}
\Delta\left(\tilde{\Gamma}\left(\vec{A};z,\tau\right)\right) = \tilde{\Gamma}\left(\vec{A};z,\tau\right) \otimes 1 + \sum_{i}\sum_{k=1}^{n-1}
\tilde{\Gamma}\left(\vec{A}_i^{(k)};z,\tau\right)\otimes [\, \Omega_i^{(n-k)} ]\, + 1 \otimes \mathbb{S}.
\ee 
The second term is given by the sum over all the terms that have an eMPL $\tilde{\Gamma}\left(\vec{A}_i^{(k)};z,\tau\right)$ of length $k$ in the first entry of the coaction and a differential $(n-k)$-form $ \Omega_i^{(n-k)}$ in the second entry, while the third term can be interpreted as the symbol of the eMPL $\tilde{\Gamma}\left(\vec{A};z,\tau\right)$ \cite{Broedel:2018iwv}. The procedure to rewrite $\tilde{\Gamma}\left(\vec{A};z,\tau\right)$ in terms of iterated integrals of modular forms is a bottom-up approach, therefore we will assume that all the eMPLs of length lower than $n$ are already expressed in terms of integrals of the kind \ref{IIh}. In the next step we focus on the third term in \ref{3TermsC}, and since it is the symbol of $\tilde{\Gamma}\left(\vec{A};z,\tau\right)$ we can integrate it and define 
\be
f_k(\tau) = \left(Id \otimes  {\scriptsize \int} \right)\Delta_{0,n}\left(\tilde{\Gamma}\left(\vec{A};z,\tau\right)\right),
\ee
where $\Delta_{i,j}$ select the terms with length $i$ and $j$ in the first and second entries of the coaction, and the integration acting on the second entry of the coaction is performed in terms of iterated integrals of modular forms. Then, by construction we have
\be
\Delta_{0,n}\left(\tilde{\Gamma}\left(\vec{A};z,\tau\right) - f_k(\tau)\right) = 0,
\ee
and so $f_k(\tau)$ encodes all the information about the terms that do not contain eMPLs in the first entry of the coaction.  Next we look at terms in the coaction with eMPLs of length 1 in the first entry. Then we can then define the quantity
\be
f_{k-1}(\tau) = f_k(\tau) + \left(Id_{IM} \otimes \int \right)\Delta_{1,n-1}\left(\tilde{\Gamma}\left(\vec{A};z,\tau\right) - f_k(\tau)\right),
\ee
where $Id_{IM}$ means that we substitute to the eMPLs in the first entry their expression in terms of iterated integrals of modular forms. As in the previous step, by construction we have
\be
\Delta_{1,n-1}\left(\tilde{\Gamma}\left(\vec{A};z,\tau\right) - f_{k-1}(\tau)\right) = 0,
\ee
which means that we have fixed also the terms with eMPLs of length 1 in the first entry of the coaction. Proceeding iteratively we are able to rewrite entirely any eMPL in terms of iterated integrals of modular forms exploiting this algorithm. As final comment we discuss how to the determine eventually boundary constants, indeed at the last step of the procedure just described we obtain
\be
\Delta\left(\tilde{\Gamma}\left(\vec{A};z,\tau\right) -f_1(\tau)\right) = \left(\tilde{\Gamma}\left(\vec{A};z,\tau\right) - f_1(\tau)\right) \otimes 1,
\ee
which implies that $\tilde{\Gamma}\left(\vec{A};z,\tau\right)$ and its expression in terms of iterated integrals of modular forms $f_1$ differs by a constant, which can be computed at the cusp at infinity $\tau_0 = i \infty$.\par
The coaction acts on \ref{Gex} as
\bea
\label{CoacGex}
\Delta\left(\tilde{\Gamma}{\scriptsize\left(\begin{array}{cc} 0 & 1 \\ 0 & \frac{2}{3}\end{array}; \frac{\tau}{2}, \tau\right)}\right) & = & \tilde{\Gamma}{\scriptsize\left(\begin{array}{cc} 0 & 1 \\ 0 & \frac{2}{3}\end{array}; \frac{\tau}{2}, \tau\right)} \otimes 1 + \tilde{\Gamma}{\scriptsize\left(\begin{array}{c} 0 \\ 0 \end{array}; \frac{\tau}{2}, \tau\right)}\otimes (T_A)_{1,2} + \tilde{\Gamma}{\scriptsize\left(\begin{array}{c} 1 \\ \frac{2}{3} \end{array}; \frac{\tau}{2}, \tau\right)}\otimes (T_A)_{1,3} \nn \\
&& + \tilde{\Gamma}{\scriptsize\left(\begin{array}{c} 2 \\ \frac{2}{3} \end{array}; \frac{\tau}{2}, \tau\right)} \otimes (T_A)_{1,4} + 1 \otimes (T_A)_{1,5},
\eea
where we assume that iterated integrals of modular forms expressions for the length one eMPLs are already been computed:
\bea
\tilde{\Gamma}{\scriptsize\left(\begin{array}{c} 0 \\ 0 \end{array}; \frac{\tau}{2}, \tau\right)} & = & \frac{1}{2}I {\scriptsize\left(\begin{array}{cc} 0 & 0 \\ 0 & 0\end{array};\tau\right)}, \nn \\
\tilde{\Gamma}{\scriptsize\left(\begin{array}{c} 1 \\ \frac{2}{3} \end{array}; \frac{\tau}{2}, \tau\right)} & = & -\frac{i \pi}{4}I{\scriptsize\left(\begin{array}{cc} 0 & 0 \\ 0 & 0 \end{array};\tau\right)} + \frac{i}{2\pi}I{\scriptsize\left(\begin{array}{cc} 2 & 6 \\ 2 & 0 \end{array};\tau\right)} - \frac{i}{2 \pi}I{\scriptsize\left(\begin{array}{cc} 2 & 6 \\ 2 & 3 \end{array};\tau\right)} - G\left(e^{-\frac{2 i \pi}{3}};1\right), \nn \\
\tilde{\Gamma}{\scriptsize\left(\begin{array}{c} 2 \\ \frac{2}{3} \end{array}; \frac{\tau}{2}, \tau\right)} & = & - \frac{\pi^2}{12}{\scriptsize\left(\begin{array}{cc} 0 & 0 \\ 0 & 0 \end{array};\tau\right)} - \frac{1}{2}{\scriptsize\left(\begin{array}{cc} 2 & 6 \\ 2 & 3 \end{array};\tau\right)} + \frac{i}{\pi}{\scriptsize\left(\begin{array}{cc} 3 & 6 \\ 2 & 0 \end{array};\tau\right)} - \frac{i}{\pi}{\scriptsize\left(\begin{array}{cc} 3 & 6 \\ 2 & 3 \end{array};\tau\right)}.
\eea
However, as already said, we only need the cusp values for the eMPLs in the first entry of the coaction:
\bea
Cusp\left(\tilde{\Gamma}{\scriptsize\left(\begin{array}{c} 0 \\ 0 \end{array}; \frac{\tau}{2}, \tau\right)}\right) & = & 0, \nn \\
Cusp\left(\tilde{\Gamma}{\scriptsize\left(\begin{array}{c} 1 \\ \frac{2}{3} \end{array}; \frac{\tau}{2}, \tau\right)}\right) & = &  - G\left(e^{-\frac{2 i \pi}{3}};1\right), \nn \\
Cusp\left(\tilde{\Gamma}{\scriptsize\left(\begin{array}{c} 2 \\ \frac{2}{3} \end{array}; \frac{\tau}{2}, \tau\right)}\right) & = & 0, \nn \\
Cusp\left(\tilde{\Gamma}{\scriptsize\left(\begin{array}{cc} 0 & 1 \\ 0 & \frac{2}{3}\end{array}; \frac{\tau}{2}, \tau\right)}\right) & = & \frac{i}{2\pi}G{\scriptsize\left(0,e^{-\frac{2 i \pi}{3}},1;1\right)}.
\eea
Therefore the explicit expression for the coaction \ref{CoacGex} is
\bea
\label{CoacGex2}
\Delta\left(\tilde{\Gamma}{\scriptsize\left(\begin{array}{cc} 0 & 1 \\ 0 & \frac{2}{3}\end{array}; \frac{\tau}{2}, \tau\right)}\right) & = & - G\left(e^{-\frac{2 i \pi}{3}};1\right) 1 \otimes \frac{d\tau}{2} - 1\otimes [\, \frac{d\tau}{2}\vert \frac{d\tau}{2 i \pi }h^{(2)}_{6,2,0}(\tau)]\, - [\,\frac{i \pi d\tau}{4}\vert \frac{d\tau}{2}]\, \nn \\
&& - [\, \frac{i d\tau}{2\pi}h^{(2)}_{6,2,3}(\tau) \vert \frac{d\tau}{2} ]\, - [\, \frac{d\tau}{2 i \pi} h^{(2)}_{6,2,0}(\tau)\vert \frac{d\tau}{2} ]\, + [\,\frac{\pi^2 d\tau}{12} \vert \frac{i d\tau}{2 \pi} ]\,  \nn \\
&&+ [\, \frac{d\tau}{2}h^{(2)}_{6,2,3}(\tau)\vert \frac{i d\tau}{2 \pi} ]\, + [\, \frac{i d\tau}{\pi} h^{(3)}_{6,2,3}(\tau) \vert \frac{i d\tau}{2 \pi} ]\, - [\, \frac{i d\tau}{\pi} h^{(3)}_{6,2,0}(\tau) \vert \frac{i d\tau}{2 \pi} ]\,. \nn \\
\eea
Finally, by integrating the second entry of the coaction\footnote{We stress that when performing integration the ordering of the differential forms in \ref{CoacGex2} is reversed.} we get the expression for $\tilde{\Gamma}{\scriptsize\left(\begin{array}{cc} 0 & 1 \\ 0 & \frac{2}{3}\end{array}; \frac{\tau}{2}, \tau\right)}$ in terms of iterated integrals of modular forms:
\bea
\tilde{\Gamma}{\scriptsize\left(\begin{array}{cc} 0 & 1 \\ 0 & \frac{2}{3}\end{array}; \frac{\tau}{2}, \tau\right)} & \cong & \frac{i}{2\pi}G{\scriptsize\left(0,e^{-\frac{2 i \pi}{3}},1;1\right)}  - G\left(e^{-\frac{2 i \pi}{3}};1\right)I{\scriptsize\left(\begin{array}{cc} 0 & 0 \\ 0 & 0 \end{array};\tau\right)} -\frac{i \pi}{12}I{\scriptsize\left( \begin{array}{cc} 0 & 0 \\ 0 & 0 \end{array} \bigg | \begin{array}{cc} 0 & 0 \\ 0 & 0 \end{array};\tau\right)} \nn \\
&& + \frac{i }{4 \pi}I{\scriptsize\left( \begin{array}{cc} 0 & 0 \\ 0 & 0 \end{array} \bigg | \begin{array}{cc} 2 & 6 \\ 2 & 0 \end{array};\tau\right)} + \frac{1}{2 \pi^2}I{\scriptsize\left( \begin{array}{cc} 0 & 0 \\ 0 & 0 \end{array} \bigg | \begin{array}{cc} 3 & 6 \\ 2 & 0 \end{array};\tau\right)} - \frac{1}{2 \pi^2}I{\scriptsize\left( \begin{array}{cc} 0 & 0 \\ 0 & 0 \end{array} \bigg | \begin{array}{cc} 3 & 6 \\ 2 & 3 \end{array};\tau\right)} \nn \\
&& \frac{i }{4 \pi }I{\scriptsize\left( \begin{array}{cc} 2 & 6 \\ 2 & 0 \end{array} \bigg | \begin{array}{cc} 0 & 0 \\ 0 & 0 \end{array};\tau\right)}.
\eea












